QuickLAP: Quick Language-Action Preference Learning for Semi-Autonomous Agents

Robots must learn from both what people do and what they say, but either modality alone is often incomplete: physical corrections are grounded but ambiguous in intent, while language expresses high-level goals but lacks physical grounding. We introduce QuickLAP: Quick Language-Action Preference learning, a Bayesian framework that fuses physical and language feedback to infer reward functions in real time. Our key insight is to treat language as a probabilistic observation over the user's latent preferences, clarifying which reward features matter and how physical corrections should be interpreted. QuickLAP uses Large Language Models (LLMs) to extract reward feature attention masks and preference shifts from free-form utterances, which it integrates with physical feedback in a closed-form update rule. This enables fast, real-time, and robust reward learning that handles ambiguous feedback. In a semi-autonomous driving simulator, QuickLAP reduces reward learning error by over 70% compared to physical-only and heuristic multimodal baselines. A 15-participant user study further validates our approach: participants found QuickLAP significantly more understandable and collaborative, and preferred its learned behavior over baselines. Code is available at https://github.com/MIT-CLEAR-Lab/QuickLAP.

==> app.tex <==

\appendix
\section{Derivations and Algorithmic Details}
\label{app:derivation}


\section{QuickLAP MAP Update Derivation}
\label{app:quicklap-map-derivation}

We base our derivation on the graphical model shown below.

\begin{figure}[ht]
    \centering
    \includegraphics[width=\linewidth]{figures/GM_QuickLAP.pdf}
    \caption{Graphical model for QuickLAP. The robot optimizes with current reward parameters $\theta^t$, which generate a candidate trajectory $\xi_R$. The human has latent true reward parameters $\theta$. An attention mask $r^t$ (at time $t$) selects the feature subspace currently attended, introducing a latent shift $\mu$ between human and robot rewards. Given $\xi_R$, the human may provide a physical intervention $\xi_H$ under $\theta$, and a language utterance $l$ that directly informs $\mu$. Shaded nodes are observed ${\theta^t, \xi_R, \xi_H, l}$; unshaded nodes are latent ${\theta, r, \mu}$.}
    \label{fig:placeholder}
\end{figure}

Starting from the posterior in Eq.~(3) of the main text:
\begin{equation}
P(\theta \mid \xi_H, \xi_R, l) \propto P(\xi_H \mid \xi_R, \theta) \cdot P(l \mid \xi_H, \xi_R, \theta) \cdot P(\theta \mid \hat{r})
\end{equation}
To deal with the infeasible $P(l \mid \xi_H, \xi_R, \theta)$, we introduce a latent shift $\mu$ that is informed by the language $l$ and conditioned on $\theta$ and $\theta^t$. We get:
\begin{equation}
P(\theta \mid \xi_H, \xi_R, l) \propto P(\xi_H \mid \xi_R, \theta) \cdot P(\mu \mid \theta, \theta^t) \cdot P(l \mid \mu) \cdot P(\theta \mid \hat{r})
\end{equation}
Since $l$ is independent of $\theta$ given $\mu$, the language term reduces to a factor over $\mu$; the prior $P(\mu \mid \theta, \theta^t)$ remains.

\para{Step 1: Log-Posterior Construction.}
Taking the logarithm and substituting our component models:
\begin{equation}
\begin{aligned}
\log P(\theta \mid \cdot)
&= \theta^\top \Delta\Phi - \lambda \|\xi_H - \xi_R\|^2 \\
&\quad - \frac{1}{2}(\theta - \theta^t)^T
\Lambda_{\text{prior}}(\hat{r}^t)(\theta - \theta^t) \\
&\quad - \frac{1}{2}(\mu^t - (\theta^t - \theta))^T
\Sigma_L^{-1}(m^t)(\mu^t - (\theta^t - \theta)) \\
&\quad + \text{const}
\end{aligned}
\end{equation}

where:
\begin{itemize}
\item $\Delta\Phi = \Phi(\xi_H) - \Phi(\xi_R)$ is the feature difference
\item $\Lambda_{\text{prior}}(\hat{r}^t) = \text{diag}(1/(\alpha(\hat{r}_i^t + \epsilon_{\text{prior}})))$ is attention-modulated precision
\item $\Sigma_L^{-1}(m^t) = \text{diag}(1/\sigma_L^2(m_i^t))$ is confidence-modulated precision
\end{itemize}

\para{Step 2: MAP Optimization.}
Taking the gradient with respect to $\theta$ and setting to zero:
\begin{equation}
\begin{aligned}
\nabla_\theta \log P(\theta \mid \cdot)
&= \Delta\Phi
 - \Lambda_{\text{prior}}(\hat{r}^t)\,(\theta - \theta^t) \\
&\quad - \Sigma_L^{-1}(m^t)\,\bigl(-\mu^t + (\theta - \theta^t)\bigr)
= 0
\end{aligned}
\end{equation}

\para{Step 3: Element-wise Solution.}
For each feature $i$, rearranging:
\begin{align}
\Delta\Phi_i &= \Lambda_{\text{prior},i}(\theta_i - \theta_i^t) + \sigma_{L,i}^{-2}(\theta_i - (\theta_i^t + \mu_i^t)) \\
\Delta\Phi_i &= (\Lambda_{\text{prior},i} + \sigma_{L,i}^{-2})\theta_i - \Lambda_{\text{prior},i}\theta_i^t - \sigma_{L,i}^{-2}(\theta_i^t + \mu_i^t)
\end{align}

Solving for $\theta_i$:
\begin{equation}
\theta_i = \frac{\Delta\Phi_i + \Lambda_{\text{prior},i}\theta_i^t + \sigma_{L,i}^{-2}(\theta_i^t + \mu_i^t)}{\Lambda_{\text{prior},i} + \sigma_{L,i}^{-2}}
\end{equation}

Simplifying to the final update rule:
\begin{equation}
\label{eq:map-update}
\boxed{\hat{\theta}_{i}^{t+1} = \hat{\theta}_i^t + \frac{\sigma_{L,i}^2 \Delta\Phi_i + \mu_i^t}{\Lambda_{\text{prior},i} \sigma_{L,i}^2 + 1}}
\end{equation}

\para{Attention-Dependent Prior Precision:}
\begin{equation}
\Lambda_{\text{prior},i}(\hat{r}_i^t) = \frac{1}{\alpha(\hat{r}_i^t + \epsilon_{\text{prior}})}
\end{equation}
where $\alpha$ is the base variance scale and $\epsilon_{\text{prior}} \ll 1$ ensures minimum precision.

\para{Confidence-Dependent Language Variance:}
\begin{equation}
\sigma_L^2(m_i^t) = k^2 \cdot \frac{(1 - m_i^t)^2}{(\epsilon_{\text{var}} + m_i^t)^2}
\end{equation}


\section{Derivation and Interpretation of the QuickLAP Update}
\label{app:quicklap_interp}
\para{Interpretation.}
Eq.~\eqref{eq:quicklap-MAP} exhibits a Kalman‐style fusion in which an \emph{attention–adaptive precision} term decides the credit assignment between modalities.  
We define the scalar gain
\[
\kappa_i(m_i^t, \hat{r}_i^t) = \bigl[\Lambda_{prior,i}(\hat{r}_i^t)\sigma_{L,i}^{2}(m_i^t)+1\bigr]^{-1}\enspace.
\]
The MAP update can be rewritten element-wise as:
\[
\hat{\theta}_i^{t+1} = \theta_i^{t} + \kappa_i(m_i^t, \hat{r}_i^t)\,\bigl[\,\sigma_{L,i}^{2}(m_i^t)\,\Delta\Phi_i+\mu_i^t\bigr].
\]
The behavior of this update depends on the attention gate $\hat{r}_i^t$ (via $\Lambda_{prior,i}$) and language confidence $m_i^t$ (via $\sigma_{L,i}^2$).
For features with high attention score (low prior precision $\Lambda_{prior,i}$) and high language confidence (low language variance $\sigma_{L,i}^2 \approx \epsilon_{var}$), $\kappa_i \approx 1$. The update is dominated by the language-suggested shift $\mu_i^t$, while the physical correction $\Delta\Phi_i$ is suppressed by the small $\sigma_{L,i}^2$ multiplier.
Conversely, if language confidence is low (large $\sigma_{L,i}^2$), then $\kappa_i \sigma_{L,i}^2 \approx 1/\Lambda_{prior,i}$. The update gives more weight to the physical correction $\Delta\Phi_i$, scaled by the prior variance. If attention score $\hat{r}_i^t$ is low (high prior precision $\Lambda_{prior,i}$), $\kappa_i$ becomes small, and $\theta_i$ changes little from $\theta_i^t$, primarily driven by $\Delta\Phi_i$ if $\mu_i^t$ is also small or language confidence is low. This adaptive weighting allows QuickLAP to react decisively to clear interventions while remaining robust to ambiguous signals.

\section{QuickLAP Algorithm}
\label{app:quicklap-algorithm}

\begin{algorithm}[H]
\caption{QuickLAP Online Learning Update \label{alg:quicklap}}
\begin{algorithmic}[1]
\Require Human correction $\xi_H$, robot plan $\xi_R$, language utterance $l$, current weights $\hat{\theta}^t$
\Ensure Updated weights $\hat{\theta}^{t+1}$

    \State Compute physical feature difference: $\Delta\Phi \leftarrow \Phi(\xi_H) - \Phi(\xi_R)$
    \State Extract attention mask: $\hat{r} \leftarrow \text{LM}_{\text{att}}\bigl(l, \Delta\Phi\bigr)$
    \State Extract preference shift and confidence: $(\mu, m) \leftarrow \text{LM}_{\text{pref}}\bigl(l, \Delta\Phi, \hat{r}\bigr)$
    \For{$i \gets 1$ \textbf{to} $d$} \Comment{$d$ is the number of features}
        \State $\Lambda_{\text{prior},i} \leftarrow \dfrac{1}{\alpha\, (\hat{r}_i + \epsilon_{\text{prior}})}$ \Comment{attention-weighted prior precision}
        \State $\sigma_{L,i}^2 \leftarrow k^2\, \dfrac{(1 - m_i)^2}{\bigl(\epsilon_{\text{var}} + m_i\bigr)^2}$ \Comment{confidence-dependent variance}
        \State $\displaystyle \hat{\theta}_i^{t+1} \leftarrow \hat{\theta}_i^{t} + \frac{\sigma_{L,i}^2 \, \Delta\Phi_i + \mu_i}{\Lambda_{\text{prior},i}\, \sigma_{L,i}^2 + 1}$ \Comment{MAP update (Eq.~\eqref{eq:map-update})}
    \EndFor
    \State \Return $\hat{\theta}^{t+1}$
\end{algorithmic}
\end{algorithm}


\section{Physical--Language Trade-off Visualization}
\label{app:tradeoff}

Figure~\ref{fig:tradeoff} illustrates the key insight of QuickLAP: as language confidence $m$ increases, the system transitions from relying primarily on physical corrections ($w_\phi$) to trusting language-suggested changes ($w_\mu$). This adaptive weighting allows QuickLAP to handle both ambiguous and precise language feedback appropriately.

\begin{figure}[H]
\centering
\includegraphics[width=\linewidth]{figures/weight_relationship_plot.pdf}
\caption{Trade-off between physical correction weight ($w_\phi$) and language guidance weight ($w_\mu$) as a function of language confidence $m$ for high attention ($r = 1.0$). When language confidence is low ($m \approx 0$), the system relies heavily on physical corrections. As confidence increases ($m \to 1$), QuickLAP shifts toward trusting the language-suggested preference changes. This smooth transition enables robust multimodal fusion.}
\label{fig:tradeoff}
\end{figure}

The mathematical relationship shown in the figure follows from our update rule:
\begin{align}
w_\phi &= \frac{\sigma_{L}^2}{\Lambda_{\text{prior}} \sigma_{L}^2 + 1} \\
w_\mu &= \frac{1}{\Lambda_{\text{prior}} \sigma_{L}^2 + 1}
\end{align}

where $\sigma_L^2(m) = k^2 \cdot \frac{(1-m)^2}{(\epsilon_{\text{var}} + m)^2}$ creates the smooth transition from physical-dominant to language-dominant updates. In this figure, $k = 1.0$ and $\Lambda_{\text{prior}} = 1.0$ (high attention, $r = 1.0$). The parameter $k$ controls the steepness of the transition: larger values of $k$ create sharper transitions around $m = 0.5$, while smaller values result in more gradual weight shifts across the confidence spectrum.

\section{Prompts, Experimental Details, and User Study Materials}
\label{app:prompts}

\section{LLM Prompt Templates}
\label{app:prompts-templates}
In this section of the appendix, we provide the full prompts that we used to query the LLMs in our studies.

\section{Attention Language Model ($\text{LM}_{\text{att}}$)}
\label{app:lm-att}

\textbf{System Message:}
\begin{lstlisting}
You are an expert in autonomous vehicle control analyzing driver interventions. In this task, a human driver has intervened to correct the behavior of a robot car and has provided an explanation of the intervention. Your task is to determine which features are relevant to a given intervention explanation, given the change in feature values of the human trajectory compared to the robot trajectory. Positive values mean that the human increased the feature value.

Note that a feature may be irrelevant even if it has a large change in value. Only output features that are relevant to the intervention explanation.

Output STRICT JSON with the single key 'gate': a list of attention gates scores (one per feature, 0.0 or 1.0). NO other keys.
\end{lstlisting}

\textbf{User Message Template:}
\begin{lstlisting}
Human Driver Intervention Explanation:
{explanation}

Current Feature Values:
- speed_desirability (How close the car's speed is to the desired speed limit): feature change after intervention: {speed_change:+.3f}, the human {speed_direction} this feature
- lane_alignment (How well the car stays centered in its lane): feature change after intervention: {lane_change:+.3f}, the human {lane_direction} this feature
- off_road (Penalty for driving off the road): feature change after intervention: {offroad_change:+.3f}, the human {offroad_direction} this feature
- cone_distance (Safe distance from traffic cones): feature change after intervention: {cone_change:+.3f}, the human {cone_direction} this feature
- car_distance (Safe distance from other vehicles): feature change after intervention: {car_change:+.3f}, the human {car_direction} this feature
- puddle_distance (Safe distance from puddles): feature change after intervention: {puddle_change:+.3f}, the human {puddle_direction} this feature

For absolutely EVERY feature above, determine:
1. How relevant is this feature to the intervention? (gate score 0.0 or 1.0)
\end{lstlisting}


\section{Preference Language Model ($\text{LM}_{\text{pref}}$)}
\label{app:lm-pref}

\textbf{System Message:}
\begin{lstlisting}
You are an expert in autonomous vehicle control analyzing driver interventions. In this task, a human driver has intervened to correct the behavior of a robot car and has provided an explanation of the intervention. Your reward function is the sum of the features. You want to maximize the reward function.

Feature values are between 0 and 1. Look at the feature descriptions to understand the scale of the features. Your task is to determine for EACH feature how much in magnitude should the weight of the feature be changed to support the intervention and human preference (mu between 0 and 6), and how confident you are in your decision (confidence between 0 and 1, be conservative), given the change in feature values of the human trajectory compared to the robot trajectory. Positive values mean that the human increased the feature value.

FOR EVERY FEATURE, return ONLY the values in this exact format.

OUTPUT (strict JSON, single line):
{
    'mu': [u1, u2, ... , uN],
    'confidence': [c1, c2, ... , cN]
}
\end{lstlisting}

\textbf{User Message Template:}
\begin{lstlisting}
Human Driver Intervention Explanation:
{explanation}

Current Feature Values:
[Same feature list as LM_att with current robot/human values]

Current Reward Weights after a Physical Intervention Update:
- speed_desirability: {current_weight_0:.3f}
- lane_alignment: {current_weight_1:.3f}
- off_road: {current_weight_2:.3f}
- cone_distance: {current_weight_3:.3f}
- car_distance: {current_weight_4:.3f}
- puddle_distance: {current_weight_5:.3f}

Now, for absolutely EVERY feature (considering the explanation, feature changes, and current weights):
1. What absolute change with direction (this will be your 'mu') would support this intervention? Consider the scale of the features, and the current weights.
2. How confident are you in your decision? (confidence score 0.0-1.0)
\end{lstlisting}


\section{LLM Configuration Parameters}
\label{app:llm-config}

The table below describes the parameters we used for the LLM experiments using the OpenAI API.

\begin{table}[h]
\centering
\caption{LLM API Configuration Settings}
\begin{tabular}{lcc}
\toprule
\textbf{Parameter} & $\textbf{LM}_{\text{att}}$ & $\textbf{LM}_{\text{pref}}$ \\
\midrule
Model & gpt-4o & gpt-4o \\
Temperature & 0.1 & 0.3 \\
Response Format & JSON & JSON \\
Max Tokens & default & default \\
\bottomrule
\end{tabular}
\end{table}


\section{User Study Questionnaire}
\label{app:user-study-questionnaire}

\begin{table*}[ht]
\centering
\caption{Questionnaire constructs, items, and reliability used in the user study, adapted from Bajcsy et al.~\cite{bajcsy2017phri}.}
\label{tbl:questions}
\begin{tabular}{p{3.5cm} p{9cm} c}
\hline
\textbf{Construct} & \textbf{Items} & \textbf{Cronbach's $\alpha$} \\
\hline
\multirow{2}{*}{Understandability}
  & The robot understood how I wanted to do the task. & \multirow{2}{*}{$\alpha=.953$} \\
  & The robot learned from my corrections. & \\
\hline
\multirow{2}{*}{Ease of Use}
  & The robot required minimal corrections. & \multirow{2}{*}{$\alpha=.816$} \\
  & (Negative) I had to keep correcting the robot. & \\
\hline
\multirow{2}{*}{Predictability}
  & It was easy to anticipate how the robot would respond to my corrections. & \multirow{2}{*}{$\alpha=.750$} \\
  & (Negative) The robot’s response to my corrections surprised me. & \\
\hline
\multirow{2}{*}{Collaborativity}
  & The robot worked with me to complete the task. & \multirow{2}{*}{$\alpha=.928$} \\
  & (Negative) The robot did not collaborate with me to complete the task. & \\
\hline
\end{tabular}
\end{table*}


\section{Additional Simulated Experiment Details}
\label{app:experiments}

In this section of the appendix, we describe the implementation details of the simulated environment that were not covered in the main text.

\subsection{Feature Definitions and Computations}
\label{app:feature-defs}

Below is a table of formulas used to calculate the features we used to represent a user's preference. Here, $\sigma$ refers to the sigmoid function.

\begin{table}[H]
\centering
\caption{Exact Feature Definitions Used in Experiments}
\begin{tabularx}{\linewidth}{
  >{\raggedright\arraybackslash}p{2cm}
  >{\raggedright\arraybackslash}X
}

\toprule
\textbf{Feature} & \textbf{Mathematical Definition} \\
\midrule
speed\_desirability & $1.0 - \left(\frac{v - v_{\text{target}}}{v_{\text{target}}}\right)^2$ \\
\addlinespace
lane\_alignment & $1-\left(\frac{d_{\text{lane}}}{\text{lane\_width}}\right)^2$ \\
\addlinespace
off\_road & $1.0$ if in bounds, else
$1.0 - \left(\frac{d_{\text{boundary}}}{\mathrm{lane\_width}}\right)^2$ \\
\addlinespace
cone\_distance &
$\min\!\left(1-\frac{r_{\text{safe}}-d_{\text{cone}}}{r_{\text{safe}}}\cdot
\sigma\!\left(-\gamma\cdot|\mathrm{horiz.\_distance}|\right)\right)$ \\
\addlinespace
car\_distance &
$\min\!\left(1-\frac{r_{\text{safe}}-d_{\text{car}}}{r_{\text{safe}}}\cdot
\sigma\!\left(-\gamma\cdot|\mathrm{horiz.\_distance}|\right)\right)$ \\
\addlinespace
puddle\_distance &
$\min\!\left(1-\frac{r_{\text{safe}}-d_{\text{puddle}}}{r_{\text{safe}}}\cdot
\sigma\!\left(-\gamma\cdot|\mathrm{horiz.\_distance}|\right)\right)$ \\
\bottomrule
\end{tabularx}
\end{table}



\subsection{Ground Truth Reward Weights}
\label{app:gt-weights}

The ground-truth reward weights define the ``optimal" behavior of the vehicle that we aim to achieve. The table below shows the values associated with each feature that we used in our experiments.

\begin{table}[H]
\centering
\caption{Ground Truth Preference Weights ($\theta^*$) for Each Scenario}
\resizebox{\linewidth}{!}{%
\begin{tabular}{lcccccc}
\toprule
\textbf{Scenario} & \textbf{Speed} & \textbf{Lane} & \textbf{Off-Road} & \textbf{Cone} & \textbf{Car} & \textbf{Puddle} \\
\midrule
C (Cone) & 5.0 & 2.5 & 20.0 & 40.0 & --- & --- \\
CP (Cone+Puddle) & 5.0 & 1.5 & 10.0 & 20.0 & --- & 1.0 \\
CPC-3 & 5.0 & 2.5 & 20.0 & 40.0 & 50.0 & 3.0 \\
CPC-4 & 5.0 & 2.5 & 20.0 & 40.0 & 50.0 & 3.0 \\
\bottomrule
\end{tabular}
}
\end{table}


\subsection{Hyperparameter Settings}
\label{app:hyperparams}

Our experiments used the following hyperparameters for running the InterACT lab driving simulator.

\begin{table}[H]
\centering
\caption{Complete Hyperparameter Configuration}
\begin{tabular}{lcc}
\toprule
\textbf{Parameter} & \textbf{Symbol} & \textbf{Value} \\
\midrule
Base learning rate & $\alpha$ & 1.0 \\
Language confidence scale & $\sigma$ & 1.2 \\
Numerical stability & $\epsilon$ & $10^{-4}$ \\
Prior stability & $\epsilon_{\text{prior}}$ & $10^{-6}$ \\
Variance stability & $\epsilon_{\text{var}}$ & $10^{-3}$ \\
Capping factor & --- & 5.0 \\
Beta power & $p$ & 2.0 \\
Simulation frequency & --- & 30 Hz \\
Planning horizon & --- & 5 timesteps \\
Episode length & --- & 220 timesteps \\
\bottomrule
\end{tabular}
\end{table}


\subsection{Computational Requirements}
\label{app:compute}

Our simulated results require the following hardware considerations to be satisfied in order to run.

\begin{table}[H]
\centering
\caption{Computational Analysis}
\begin{tabular}{lc}
\toprule
\textbf{Metric} & \textbf{Value} \\
\midrule
Hardware & CPU \\
Per-episode runtime & $\sim$1 minute \\
LLM API calls per intervention & 2 (LM$_{\text{att}}$ + LM$_{\text{pref}}$) \\
Storage per experiment & $<$2MB (logs + trajectories) \\
\bottomrule
\end{tabular}
\end{table}


\subsection{Natural Language Utterances}
\label{app:utterances}

The five natural language utterances used across all experiments, ordered by specificity:

\begin{enumerate}
\item \textbf{"Be careful."} (most ambiguous)
\item \textbf{"Watch out for that thing."} (moderate ambiguity)
\item \textbf{"Stay away from that thing."} (moderate specificity)
\item \textbf{"Avoid the obstacle."} (specific action)
\item \textbf{"Stay away from construction zones."} (specific action)
\item \textbf{"Steer clear of the cone."} (most specific)
\end{enumerate}


\subsection{Intervention Configuration}
\label{app:interventions}

\textbf{Intervention Windows:} Human interventions in our simulated experiments occur during these timestep ranges:
\begin{itemize}
\item Intervention 1: timesteps 45--55
\item Intervention 2: timesteps 85--95
\item Intervention 3: timesteps 130--140
\item Intervention 4: timesteps 170--180
\end{itemize}

\textbf{Correction Generation:} Simulated human trajectory generated by running the planner with the ground truth preference weights.


\subsection{Critical Implementation Details}
\label{app:impl-details}

\textbf{$\mu$ Capping Mechanism:} To prevent instability, LLM-generated preference shifts are capped:
\begin{equation}
\mu_i^{\text{capped}} = \text{sign}(\mu_i) \cdot \min(|\mu_i|, 5.0 \cdot |\Delta\Phi_i|)
\end{equation}

\textbf{Feature Normalization:} Features are normalized such that their highest value is 1 and they decrease to approximately 0 in undesirable situations.


\subsection{Per-Scenario Performance Breakdown}
\label{app:scenario-breakdown}

We reported aggregated NMSE scores in the main text. Here we provide the marginal NMSE values for each environment and each baseline in our simulated experiments.

\begin{table}[H]
\centering
\caption{Normalized MSE by Scenario (mean $\pm$ SEM across 6 utterances for 4 intervention experiment)}
\resizebox{\linewidth}{!}{%
\begin{tabular}{lccc}
\toprule
\textbf{Scenario} & \textbf{Physical-Only (pHRI)} & \textbf{Masked dPhi} & \textbf{QuickLAP} \\
\midrule
C (Cone) & $0.6923 \pm 0.0000$ & $0.4783 \pm 0.0116$ & $\mathbf{0.2071 \pm 0.0453}$ \\
CP (Puddle) & $0.5941 \pm 0.0013$ & $0.3034 \pm 0.0236$ & $\mathbf{0.0761 \pm 0.1090}$ \\
CPC-3 & $0.4496 \pm 0.0000$ & $0.4177 \pm 0.0004$ & $\mathbf{0.3468 \pm 0.0331}$ \\
CPC-4 & $0.3189 \pm 0.0000$ & $0.2876 \pm 0.0003$ & $\mathbf{0.2058 \pm 0.0525}$ \\
\bottomrule
\end{tabular}
}
\end{table}


\subsection{Language Robustness Analysis}
\label{app:language-robustness}

We performed an analysis of different kinds of feedback that a person may provide in simulation to test the robustness of our approach to different ways of communicating with the vehicle.

\begin{table}[t]
\centering
\resizebox{\linewidth}{!}{%
\begin{tabular}{lccc}
\toprule
\textbf{Utterance$^\dagger$} & \textbf{Masked} & \textbf{QuickLAP} & \textbf{pHRI} \\
\midrule
Avoid obstacle & $0.3687$ & $\mathbf{0.1877}$ & $0.5137$ \\
Be careful & $0.3870$ & $\mathbf{0.2772}$ & $0.5137$ \\
Stay away (construction) & $0.3687$ & $\mathbf{0.2087}$ & $0.5137$ \\
Stay away (object) & $0.3687$ & $\mathbf{0.2068}$ & $0.5137$ \\
Steer clear (cone) & $0.3687$ & $\mathbf{0.1672}$ & $0.5137$ \\
Watch out (object) & $0.3687$ & $\mathbf{0.2062}$ & $0.5100$ \\
\bottomrule
\end{tabular}}
\caption{NMSE across methods for different natural language utterances.
$^\dagger$Utterances abbreviated; full forms provided in text.}
\label{tab:utterance_nmse}
\end{table}

\begin{figure}[t]
  \centering
  \subfloat[Performance with ambiguous utterances]{%
    \includegraphics[width=0.23\textwidth]{results/weights_mse_grouped_no_context.png}%
    \label{fig:no_context_language_only_results}%
  }\hspace{0.01\textwidth}
  \subfloat[Robosuite Simulation]{%
    \includegraphics[width=0.23\textwidth]{RSS2026/results/robosuite_simulated_results.png}%
    \label{fig:arm_sim_results}%
  }
\end{figure}


\subsubsection{Follow-Up: Ambiguous Language Without Physical Grounding}
\label{subsubsec:ambiguous_language_no_context}

To better understand how language-driven reward updates behave under realistic ambiguity, we performed a follow-up simulation study focusing on underspecified and context-dependent language.
In the simulated experiments above, language inputs were designed to clearly reflect feature-level intent (e.g., ``avoid the cone'').
However, in practice, language feedback may be high-level, ambiguous, or context-dependent, such as utterances like ``Move.'' or ``Uhh...''.
We use the \textbf{QuickLAP No Context Language Only:} This ablation removes the physical-intervention context from the LLM input, so the language model must interpret the utterance without any grounding from the observed correction. Comparing against the contextual \textit{QuickLAP Language Only} condition isolates the importance of grounding language interpretation with physical feedback information.
While QuickLAP is designed to interpret such utterances using feature-level intervention context from the physical correction, this raises an important question:
\emph{what happens if the language model is asked to interpret ambiguous statements without any physical grounding in its context window?}

\paragraph{Setup.}
We selected a subset of ambiguous natural-language utterances and replayed them in simulation across the same driving environments described in Section~\ref{subsec:exp}.
We compare our full method (QuickLAP) against the physical-only baselines (pHRI and Masked pHRI), the contextual \textit{QuickLAP Language Only} condition, and a new ablation we call \textit{QuickLAP No Context Language Only}, as defined in Section~\ref{subsec:exp}.
In this ablation, the language model receives only the raw utterance, without any physical-intervention context or feature-level grounding, and the resulting update is driven solely by the language-implied shift.

\paragraph{Results.}
Figure~\ref{fig:no_context_language_only_results} shows that removing physical grounding from the LLM input degrades performance.
The \textit{QuickLAP No Context Language Only} baseline exhibits the highest normalized reward-weight MSE across all environments compared to other QuickLAP variants, which perform comparably to earlier results in Figure~\ref{fig:mse_across_envs}.
This pattern suggests that the primary failure mode of language-only learning is not simply the absence of a physical term in the Bayesian update, but the absence of physical grounding \emph{in the language interpretation process itself}.

\paragraph{Takeaway.}
These findings highlight the importance of grounding language in physical interaction.
Language alone is often ambiguous and underspecified, and without shared situational context it can induce large, misaligned updates.
Physical corrections provide a crucial grounding signal that anchors linguistic intent to concrete, feature-level consequences.
QuickLAP exploits this complementarity by using language to specify what should change and physical corrections to ground how it changes in feature space.

\section{Additional User Study Details}
\label{appendix:user_study_details}

We present the additional user study details here to enable future research to replicate our findings.

\textbf{Equipment.}
Participants controlled the robot using the Logitech steering wheel controller with three pedals. Participants were instructed to use the wheel as well as the gas pedal and brake pedal to control the vehicles behavior. The simulated environment was run using the CPU of a single laptop. Participants' voice commands were recorded using the laptop's built-in microphone, and were transcribed using the OpenAI Whisper speech recognition model.

\textbf{Questionnaire.}
Our user study adapted the questionnaire from Bajcsy et al.~\cite{bajcsy2017phri} with small modifications. The exact Likert items used in the study are described in Tbl.~\ref{tbl:questions}. Each question was rated on a seven-point scale from strongly disagree to strongly agree. We additionally provide the interrater reliability scores for each construct as found in our study.

In addition to the Likert questions, we asked users to rank all three algorithms that they experienced in a forced-choice ranking question. Participants were not allowed to specify that two algorithms tied. This question was phrased as ``Please use the algorithm codes (1,2,3) to rank the algorithms'' and participants were provided with three boxes arranged vertically to place the numbers one through three. The top box was labeled ``Most Preferred'' and the bottom box was labeled ``Least Preferred''.

Participants were also provided a space to take notes on each of the three algorithms. These results were not analyzed in this paper, but allowed participants to keep track of the impressions of the three algorithms throughout the study.

Following the experiment, participants were compensated with a 15 USD Amazon gift card. The entire experiment took approximately 30 minutes. 
